Relativistic limits on quantum operations

In this essay, we explore the limits imposed by the impossibility of superluminal signalling on the class of physically realisable quantum operations, focusing on the difference in approaches one can take towards this problem in Hilbert space quantum theory and algebraic quantum field theory (AQFT). We review a recent proposal by Fewster and Verch for a generally covariant measurement scheme in AQFT, which we call the FV scheme; along the way, we argue that the framework as set up in its original proposal can be greatly simplified without losing generality or physical motivation. We then discuss the problem, introduced by Sorkin, that naive generalisations of the notion of operation to the relativistic context can lead to signalling between spacelike observers by introducing a third observer. We consider approaches to tackle this problem in Hilbert space quantum theory and argue that these are sometimes ambiguous, since the physical (im)possibility of operations depends in part on the specific spacetime embodiment of the quantum system under consideration, which lies outside the Hilbert space formalism. In the AQFT context, we review and generalise a recent result showing that operations induced by the FV measurement scheme do not enable superluminal signalling. We connect this result to Hilbert space by introducing a concrete model of AQFT, which we call the `hybrid model' as it provides a way to explicitly embed Hilbert space quantum theory into spacetime using the formalism of AQFT. Finally, we show that in this model, under suitable necessary and sufficient conditions, the converse result also holds: every operation that does not enable superluminal signalling can be implemented in the FV framework.

==> sections/old/acausal-impossible.tex <==
\subsection{Will almost remove this}\label{sec:acausal-impossible}
It is questionable whether \cite{BGNP01}'s `acausal' operators are really impossible and whether superluminal signalling can always be extracted from them. For maybe it is not always possible to place Alice and Charlie around Bob such that Alice has access to system A and Charlie to system C so as to enable A to signal to C while they are still spacelike\todow{obviously, improve this sentence}. Basically, an operation should be impossible if it allows superluminal signalling in a Sorkin-like scenario. But if that is the case (that it allows superluminal signalling in such a scenario), then it doesn't automatically mean that the \emph{operation} itself is impossible; because the operation is only one of the ingredients that goes into the Sorkin scenario---one also needs the agents who signal.

For example: maybe an `acausal mmt' (\eg\ incomplete Bell mmt) is sometimes possible to achieve by Bob alone, but then the photons/electrons/qubits are so `close together' that Alice and Bob can't each have their own half while being spatially separated.

If this is indeed the case (that physical possibility of an operation depends on the precise embedding in spacetime), then we have even less hope of unifying the results of \cite{BFR21} and \cite{BGNP01}, since some (what \cite{BGNP01} call) `acausal' measurements might be possible in the FV framework; the theorem of \cite{BFR21} doesn't rule out those measurements, because it is simply impossible to extract \emph{superluminal} signalling from them.

This ties into a more general `inconvenience' of \cite{BGNP01}, which is that their approach (basically: using Hilbert spaces) assumes no specific spacetime configuration. If you `embed' their nonrelativistic Hilbert space considerations `into' an actual, relativistic, physical situation, then a (nonrelativistic) CPTP map might have multiple different possible realisations, some of which are possible and others of which are not---this I expect, but I have to think of some examples. From that point of view it will also be difficult to connect \cite{BGNP01} and \cite{BFR21}, since the idea of \cite{BFR21} is that it precisely delineates the possible operations.

\

A further weakness of \cite{BGNP01} in addressing the problem of delineating the class of physical operations: Naively, the class of 'physical (bipartite) operations' is expected to lie somewhere in between the causal and localisable operations. But that is not true, because not every localisable operator is physical---one doesn't need FV for that, it simply follows if you let one of the factors in the tensor product representing the localisable operation be itself an acausal operation (hence further subdividing the Hilbert space)\todow{ explain this further}. Indeed, the physical operations do not fit into the hierarchy they present.\todow{Explain what mean by physical}

==> sections/old/bfr-bgnp.tex <==
\section{When \textcite{BFR21} meet \textcite{BGNP01}}\label{sec:bfr-meet-bgnp}

\subsection{Causality}
What can we say about the implications of \textcite{BFR21} for the notion of ‘(semi)causality’ as in \textcite{BGNP01}, by carrying over definitions between the frameworks?

Let's first define semicausality in the tensor product framework. \todow{Stress that we don't make assumptions about causal configuration here (except that AC happens after A...). The question is simply whether $A$ can communicate to $C$ \emph{solely} by her $\L_A$---and that's why we don't allow communication of here classical mmt outcome (hence $\L_A$ nonselective).}

\begin{definition}%\label{def:semicausal}
    Let $\H_{AC} = \H_A \tns \H_C$ be finite-dimensional. An operation $\L_{AC}: \B(\H_{AC}) \to \B(\H_{AC})$ is called \defn{semicausal} or \defn{no-signalling-from-$A$-to-$C$} if for all nonselective operations (\ie\ linear CPTP maps) $\L_A: \B(\H_A)\to\B(\H_A)$ and all initial states $\rho_{AC}\in\D(\H_{AC})$, we have
    \begin{equation}
        \Tr_A \L_{AC}(\rho_{AC}) = \Tr_A \L_{AC}(\L_A\tns\id_C(\rho_{AC})).
    \end{equation}\todo{\textcite{BGNP01} normalise both sides of this equation, but I don't think that will be necessary in my discussion.} \todow{Maybe change to `no-signalling-from-$\H_A$-to-$\H_C$.}
\end{definition}

Intuitively, $\L_{AC}$ cannot be used by Alice (in possession of system $A$) to signal to Charlie (in possession of system $C$), that is, the reduced state of system $C$ is unaffected by any operation $\L_A$ on Alice's side before $\L_{AC}$ happens. (Indeed, $\L_{AC}$ should not be thought of as being `applied' by Alice and Charlie; for now, just assume that it somehow `happens'.) Note that Alice's operation $\L_A$ is restricted to trace-preserving maps; this corresponds to the fact that we don't allow Alice to communicate any classical outcome of a measurement to Charlie. \todow{Explain why not. Schrödinger's 1935 `schoolboy under examination'.}

However hideous, we prefer the terminology `no-signalling-from-$A$-to-$C$' to `semicausal', because Definition~\ref{def:semicausal} is asymmetric in $A$ and $C$; moreover, no assumption about the causal ordering or relative positions of $A$ and $C$ in spacetime is made at this stage, which use of the term `semicausal' would suggest.

Finally, note that Definition~\ref{def:semicausal} is equivalent to the one given in \textcite{BGNP01}, partly due to their Theorem~1. \todow{Expound on this}

\

Using Proposition~\ref{prop:dh-sbh} and the subsequent discussion to translate Definition~\ref{def:semicausal} into the language of states on the algebras of observables, we find:
\begin{proposition}\label{prop:semicausal-heisenberg}
    With $\H_{AB}$ as in Definition~\ref{def:semicausal}, an operation $\L_{AC}: \B(\H_{AC})\to\B(\H_{AC})$ is no-signalling-from-$A$-to-$C$ if and only if there is a map $\Gamma:\B(\H_C)\to\B(\H_C)$ such that
    \begin{equation}
        \L_{AC}^*(\one_A\tns c) = \one_A\tns\Gamma(c) \quad \text{ for all } c\in\B(\H_C);
    \end{equation}
    where $\L_{AC}^*$ is the Hilbert-Schmidt adjoint of (you guessed it) $\L_{AC}$. If this is the case, $\Gamma$ is CP, and it is unital iff $\L_{AC}$ is TP.
\end{proposition}
\begin{proof}
    \todo{Not yet LaTeXified, see pp6-7 of notes.}
\end{proof}
% Intuitively, if the transformation $\L_{AB}^*$ preserves observables of the form $\one_A\tns c$, then a unital transformation $\L_A^*$ applied by Alice does not influence Charlie's observable; conversely, ?

\

Let's now make an analogous \todow{(analogous to Def ...?)} no-signalling definition in the AQFT framework.

\begin{definition}\label{def:aqft-no-signalling}
    Let $O_A$ and $O_C$ be two spacetime regions. An operation $T:\S(\Af(M))\to\S(\Af(M))$ between states is called \defn{no-signalling-from-$O_A$-to-$O_C$} if for all operators $T_A: \S(\Af(M))\to\S(\Af(M))$ local to $O_A$ and all states $\om : \Af(M)\to\C$,
    \begin{equation}
        T\circ T_A(\om)(c) = T(\om)(c) \text{\quad for all } c\in\Af(O_C).
    \end{equation}
\end{definition}

\todow{\begin{conjecture}
    If $O_A$ and $O_C$ overlap, then either all $\tilde\L$ are \emph{signalling}-from-A-to-C, or there is at least one such $\tilde\L$. Would be nice if I could explicitly show something like that.
    
    What about the case when $O_A$ and $O_C$ are (partly) in each other's future/past lightcone?
    
    Probably state somewhere that I won't be bothered about such cases in the main text but will discuss it briefly in the discussion.
\end{conjecture}}

We can then conclude from \textcite[Theorem~2]{BFR21}:
\begin{corollary}\label{cor:bfr}
    Let $O_{A,B,C}\subseteq M$ be precompact regions such that $O_A \precsim O_B$, $O_B \precsim O_C$ and $O_A\spacelike O_C$. Causal factorisation \todow{Define this and cite relevant papers+equations} implies that any FV-induced-in-$O_B$ operation is no-signalling-from-$O_A$-to-$O_C$. \todow{Is precompactness really required for all three sets? See Lemma 3 of BFR21. And: is $O_B$ really required to have the relations specified?}
    
    \todow{Causal factorisation is really only well-defined when restricting Alice's operation to FV mmts. Find a way around this. (Just extend defn of causal factorisation?}
\end{corollary}
Note that this is actually stronger than Theorem~2 of \textcite{BFR21}: in particular, it is sufficient that Alice's operation is local to the (precompact) region $O_A$; it need not be FV-induced.

\todo{It would be nice to compare Definition~\ref{def:aqft-no-signalling} to Proposition~\ref{prop:semicausal-heisenberg}, in order to compare Corollary~\ref{cor:bfr} and Definition~\ref{def:semicausal} even more closely. For this we would need to translate the state update rule of \textcite{FV20} to the Heisenberg picture, \ie\ find an operator $\Gamma:\Af(M)\to\Af(M)$ on observables such that \[ \om'(a) = \om(\Gamma(a)) \quad\text{ for all } a\in\Af(M), \] where $\om'$ is the updated state after (nonselective) measurement in the FV framework. However, even if such a $\Gamma$ does exist, it might not admit a straightforward expression and hence not be insightful. (It exists if we make the assumption that the algebra $\Af(M)$ `is separated by its states', which \eg\ \textcite[Thm~1]{Few20} does. How legitimate is this assumption?) So in hindsight proving Prop~\ref{prop:semicausal-heisenberg} might not have been very useful.}

% \todo{It would be very nice if I could eventually show that the class of FV-induced operations is somewhere in between the causal operations and the localisable operations, thereby placing it in the hierarchy of operations presented in the conclusion of \textcite{BGNP01}. But again, to fully achieve this, we would need an equivalence between the commuting operators and Hilbert space tensor product formulations of locality. How close can I come? Maybe the closest I can come is by redefining (semi)causality and (semi)localisability in AQFT (as \eg\ Def~\ref{def:aqft-no-signalling}). Alternatively (additionally), I could try giving some examples: an example of a localisable Hilbert space operator (\eg\ nonselective complete Bell mmt), showing/arguing that its AQFT version is implementable by FV measurements; and/or an example of an acausal operator (\eg\ Sorkin's $\proj{\phi^+}$ projection), showing/arguing that it cannot be implemented in the FV framework. BUT, considering the last example: see section~\ref{sec:acausal-impossible}...}

\input{sections/acausal-impossible}



\todow{
\subsection{Localisability}
\textcite{BGNP01} define:
\begin{definition}
    Let $\H_{AB} = \H_A \tns \H_B$. Call an operation $\L : \B(\H_{AB}) \to \B(\H_{AB})$ \mbox{\defn{$\H_A$-$\H_B$-localisable}} if there are operators $\L_A:\B(\H_A)\to\B(\H_A)$ and $\L_B:\B(\H_B)\to\B(\H_B)$ such that $\L = \L_A\tns\L_B$.
\end{definition}

Analogously, in AQFT it would be logical to define localisability as

...

\todo{But it isn't clear to me that two localisable operators on spacelike regions commute...}

Anyway, it is clear that it is NOT true that all FV-induced-in-$O_1\cup O_2$ operations are $O_1$-$O_2$-localisable: some local operations are simply impossible in FV framework (e.g. Bob-measurements??).




Find out and explain why the proof of BFR21 does/doesn't work for \textit{local} operations instead of FV-induced operations.

}

==> sections/old/questions.tex <==
\section{Some questions}
\begin{itemize}
    \item \textcite{BGNP01}, on page 6, upper right column, discuss how to implement nonselective complete Bell measurement. I was planning to take this as my example of a localisable operator and try to show/argue that it can be implemented in the FV framework. However, I am not fully convinced that this protocol indeed yields Bell measurement. The operator $\mathcal E$ acts as it should, but if you condition on the shared bit string of Alice and Bob, you don't get a Bell state, but rather just the original state with a flipped sign...
    
    % In the limit of repeated trials, the result averages out to nonselective Bell measurement---but is that limit relevant in the context of superluminal signalling? We want Charlie to immediately know what message Alice has sent...
    
    \item In the FV framework, the state update of a nonselective mmt doesn't depend on the probe observable being measured. However, how about complete vs incomplete measurements? Shouldn't these lead to different state updates, even if both are nonselective?
\end{itemize}

==> titlepage-boring.tex <==
\begin{titlepage}
    \newgeometry{top=4cm,bottom=4cm,left=2cm,right=2cm,marginparwidth=1.75cm}
    
    \center
    \large

    % \includegraphics[width=.3\textwidth]{cam_logo.jpg}\\[2cm]
    
    \makeatletter
    {\sffamily\huge Relativistic limits on quantum operations}\\[3cm]
    \makeatother
    
    % {\Large\textsc{Part III Essay}}\\[3cm]
    
    % {\Large \textsc{Tein van der Lugt}}\\[0.5cm]
    
    % Department of Applied Mathematics and Theoretical Physics\\
    % Wolfson College\\
    % University of Cambridge\\ \vfill
    
    % \emph{Essay setter:}\\[0.3cm]
    % Dr \textsc{Jeremy Butterfield}\\ \vfill
    % \makeatletter
    % {\large \@date}
    % \makeatother

    % ------- Logo -------
    %\includegraphics{logo.png}\\[1cm] % Requires graphicx package

    \vfill
\end{titlepage}
